Learning by non-interfering feedback chemical signaling in physical networks

Both non-neural and neural biological systems can learn. So rather than focusing on purely brain-like learning, efforts are underway to study learning in physical systems. Such efforts include equilibrium propagation (EP) and coupled learning (CL), which require storage of two different states-the free state and the perturbed state-during the learning process to retain information about gradients. Inspired by slime mold, we propose a new learning algorithm rooted in chemical signaling that does not require storage of two different states. Rather, the output error information is encoded in a chemical signal that diffuses into the network in a similar way as the activation/feedforward signal. The steady state feedback chemical concentration, along with the activation signal, stores the required gradient information locally. We apply our algorithm using a physical, linear flow network and test it using the Iris data set with 93% accuracy. We also prove that our algorithm performs gradient descent. Finally, in addition to comparing our algorithm directly with EP and CL, we address the biological plausibility of the algorithm.

==> draft.tex <==
\section{Introduction - Backup version}

What are the basic ingredients that biological learning systems, such as brain, slime mold etc, must have? Biological systems adapt to the external environment by tailoring specific responses for given external conditions. As the system experiences enough external conditions of similar kind, it develops functionality to respond to the stimulus in a way that increases its chances of survival. In nature it is observed that this functionality is an emergent phenomenon caused due to  local interactions between components\cite{Sumpter2006}. For example, when birds come together in a  flock, they increase their chances of survival\cite{Beauchamp2021}. This happens not because of a ‘supervisor’ that commands each bird to fly in a particular way, but because these birds have special local interaction rules that give rise to emergent functionality\cite{Cucker2008}. \\ \\
In the context of neural networks\cite{nielsenneural}\cite{Yang2020}, functionality is achieved by modifying weights and biases to minimise a certain cost function. Of the many ways to do so, the algorithm of choice is the backpropagation algorithm\cite{Rumelhart1986}, which updates the network such that its weights (and biases) do gradient descent in the cost function landscape. Looking at the complex nature of the tasks that neural nets are capable of, it is possible that even biological systems achieve functionality by optimizing some cost functions by gradient descent\cite{Lillicrap2020}. Also, the long process of evolution may have optimised the ``learning algorithm" in such biological systems to update its components via gradient descent. Summing up, the ingredients for a biological learning system (BLS) should be :
\begin{enumerate}
    \item A local learning algorithm 
    \item It should minimise some cost function via gradient descent
    \item The implementation of such algorithm should be physical
\end{enumerate}
There have been myriad scholarly attempts to construct learning algorithms within physical systems\cite{Hopfield1984}\cite{Movellan1991}\cite{Pineda:1987dx}\cite{lecun1986}\cite{Richards2019}\cite{Pozzi2018}. The success of backpropagation in machine learning and the similarities between deep nets and the visual cortex\cite{Issa2018}\cite{Kriegeskorte2015}\cite{D1988}\cite{Roelfsema2018} have encouraged a search for biologically plausible learning rules analogous to backpropagation\cite{WHITTINGTON2019235}\cite{NEURIPS2020_fec87a37}\cite{Lillicrap2020}. We will focus on recent works done by B. Scellier et al\cite{Scellier2017}\cite{scellier2020deep} where they introduced "equilibrium propagation", and by M. Stern et al\cite{Stern2021}, where they introduced "coupled learning". In these models, the error information corresponding to each component is encoded in terms of difference of local physical quantities taken between two phases. At each step of training, the outputs of the network are nudged towards the target output by applying additional boundary conditions at the output nodes. Next, the system is allowed to settle to a new steady state (called ``nudged state" or ``clamped state") which is slightly better than the initial ``free state". In the limit where this nudge amplitude goes to zero, the difference of local physical quantities between these two phases encodes the gradient information\cite{Scellier2017}. Unlike the backpropagation algorithm, these algorithms achieve gradient descent without explicit top down transfer of error information.\\ \\
In our work, we present a new algorithm and a new learning rule, with two important contributions :- A) We avoid a nudged phase and show that its functionality can be realised in biology using chemical signals B) We show that our learning rule computes the gradient information locally without the need for a small nudge limit. Our inspiration comes from a structurally simple - yet functionally complex organism named Physarum polycephalum. This organism is capable of myriad complex tasks - precisely coordinating flows in its body\cite{Boussard2021}, navigating maze\cite{slimemaze2000}, connecting food sources with optimal paths\cite{tero2010}\cite{Tero2008} etc. K. Alim et al showed that a lot of these complex phenomenon can be explained by a mechanism of signal propagation\cite{Alim2017}. This organism uses a chemical signal to send information (eg; about location of food sources) across its body which triggers a change in its structure (that optimises the connection between food sources). We show in section~\ref{sec:related-work} how a similar chemical signaling mechanism can be used to realise the nudged states. \\ \\

We use this inspiration to construct a biological learning system that uses chemical signals to send error information across its body. Our system is a flow network, with node pressures \textbf{v} and pipe conductance described by weights \textbf{w}. The information from the external environment is input into the system by fixing the boundary conditions \textbf{I} at input nodes. Node pressures \textbf{v} are the non-trainable variables of the system that are determined by Laplace's equation and input boundary conditions. The functionality we want is desired pressures (``target pressures'') at output nodes for a given input \textbf{I}. To achieve this, a chemical  is released into the flow network by fixing the chemical currents at output nodes. The value $\boldsymbol{\epsilon}$ of these chemical currents is proportional to the difference between target pressures and output pressures. The chemical concentrations \textbf{u} at internal nodes are determined by the same Laplace equation, but with feedback boundary conditions $\boldsymbol{\epsilon}$.  We show that this chemical concentration \textbf{u} along with the node pressures \textbf{v} locally encode the weight gradients of the cost function that we want to optimize. We propose a new learning rule that updates the trainable weights \textbf{w} such that it does gradient descent in the cost function landscape.







\section{Vidyesh's Proof}

Now we prove our claim that the learning rule \eqref{eq:learning-rule} performs gradient descent. We must show that
\begin{equation}
    \label{eq:proof-0}
    \Delta w_{xy} = - \eta \sum_{i=1}^{p} (v(o_i^+,o_i^-)-v_d(o_i^+,o_i^-))  \dfrac{\partial v(o_i^+,o_i^-)}{\partial w_{xy}}.
\end{equation}
We need to send this information to every edge $w_{xy} \in W$. For that, we need to find $\dfrac{\partial v(o_i^+,o_i^-)}{\partial w_{xy}}$ in terms of local physical quantities defined at edge $w_{xy}$. We know that\cite{Curtis}\cite{SpielmanDanielA.2019} :
\begin{equation}
\left( \begin{array}{c}
\hat{L}
\end{array} \right)
%
\left( \begin{array}{c}
v(b_j^+) \\
v(b_j^-) \\
\vdots \\
v(o_i^+) \\
v(o_i^-) \\
\vdots \\
v(x)   \\
v(y)   \\
\end{array} \right)
=
\left( \begin{array}{c}
I_j    \\
-I_j   \\
\vdots \\
0      \\
0      \\
\vdots \\
0      \\
0      \\
\end{array} \right),
\end{equation}
where $\hat{L}$ is the graph Laplacian. Now we take the partial derivative of the above equation with respect to $w_{xy}$. The above equation is a linear system of equations stating the current conservation at every node $\{b_j^+,b_j^-,..,o_i^+,o_i^-,..,x,y,\}$. For every node $x$, denoting $e(x)$ the external current going into node $x$, we have \begin{equation}
    v(x)\sum_{y \sim x} w_{xy} - \sum_{y \sim x}v(y)w_{xy} = e(x),
\end{equation}
where $y \sim x$ denotes that $x$ and $y$ are neighbours. Taking derivative of the above equation with respect to $w_{xk}$ where $k \in \{y:y \sim x\} $ we get :
\begin{equation}
    \label{eq:proof-1}
    (\partial_{xk}v(x))\sum_{y \sim x} w_{xy} - \sum_{y \sim x}(\partial_{xk}v(y))~w_{xy} = v(k)-v(x)=v(k,x)
\end{equation}
Using this we can write:
\begin{equation}
\left( \begin{array}{cc}
\hat{L}
\end{array} \right)
%
\left( \begin{array}{c}
\partial_{xy}v(b_j^+) \\
\partial_{xy}v(b_j^-) \\
\vdots              \\
\partial_{xy}v(o_i^+) \\
\partial_{xy}v(o_i^-) \\
\vdots              \\
\partial_{xy}v(x)   \\
\partial_{xy}v(y)   \\
\end{array} \right)
=
\left( \begin{array}{c}
0       \\
0       \\
\vdots  \\
0       \\
0       \\
\vdots  \\
v(y,x)  \\
-v(y,x) \\
\end{array}  \right)
\end{equation}
Note that the external current is independent of the weights of the network. The RHS of Eq.~\ref{eq:proof-1} is simply zero if the weight $w_{xk}$ does not appear in the sum  $\sum_{y \sim x} w_{xy}$. For weight $w_{xy}$ it happens everywhere except at nodes $x$ and $y$. Using above equation we can write :
\begin{equation}
    \label{eq:proof-2}
    \partial_{xy}v(o_i^+,o_i^-) = (\delta_{o_i^+}-\delta_{o_i^-})^T L^+(\delta_{x}-\delta_{y})v(y,x),
\end{equation}
where $L^+$ is the Moore-Penrose pseudo-inverse of $L$. Here $\delta_{x}$ is the column vector such that $\delta_{x}[x]=1$ and $\delta_{x}[k]=0$ for every $k \neq x$.
%\cite[p. 101]{SpielmanDanielA.2019}
Equation~\ref{eq:proof-2} tells us how sensitive is the output $v(o_i^+,o_i^-)$ to changes in the weight $w_{xy}$. We use this property to construct a feedback mechanism where this error information is sent to weight $w_{xy}$. We release the feedback chemical at output nodes: for each pair of output nodes $(o_i^+,o_i^-)$, a current $\epsilon_i$ flows into the network through node $o_i^+$ and flows out of the network through node $o_i^-$. The steady state chemical concentration satisfies Laplace's equation:
\begin{equation}
\left( \begin{array}{cc}
\hat{L}
\end{array} \right)
%
\left( \begin{array}{c}
u(b_j^+) \\
u(b_j^-) \\
\vdots \\
u(o_i^+) \\
u(o_i^-) \\
\vdots \\
u(x)   \\
u(y)   \\
\end{array} \right)
=
\left( \begin{array}{cc}
0           \\
0           \\
\vdots      \\
\epsilon_i  \\
-\epsilon_i \\
\vdots      \\
0           \\
0           \\
\end{array} \right)
\end{equation}
Using the above equation we can write :
\begin{equation}
    \label{eq:proof-3}
    u(x,y)= \sum_{i=1}^p (\delta_{x}-\delta_{y})^T L^+(\delta_{o_i^+}-\delta_{o_i^-})\epsilon_i
\end{equation}
The pseudo-inverse of a symmetric matrix is symmetric. Therefore $L^+$ is symmetric and we can write:
\begin{equation}
    \label{eq:proof-4}
    (\delta_{x}-\delta_{y})^T L^+(\delta_{o_i^+}-\delta_{o_i^-})=(\delta_{o_i^+}-\delta_{o_i^-})^T L^+(\delta_{x}-\delta_{y})
\end{equation}
Using Eq~\ref{eq:proof-4}, \ref{eq:proof-3} and \ref{eq:proof-2} we get :
\begin{equation}
    \label{eq:proof-5}
     u(x,y)v(y,x)= \sum_{i=1}^p \epsilon_i ~ \dfrac{\partial v(o_i^+,o_i^-)}{\partial w_{xy}}
\end{equation}
Comparing Eq.~\ref{eq:proof-0} with the above equation, if we set $\epsilon_i=  \eta (v(o_i^+,o_i^-)-v_d(o_i^+,o_i^-))$, the RHS of the above equation becomes the derivative of the cost function.
Hence the learning rule $\Delta w_{xy} = u(x,y)v(x,y)$ corresponds to one step of gradient descent.



\section{Related Work}

Now we repackage our model using the language of free and nudged states. We make the following changes :
\begin{enumerate}
    \item We want the feedback current to nudge the free state output $v(o_i^+,o_i^-)$ towards the desired output $v_d(o_i^+,o_i^-)$. Note that our choice of feedback current $\epsilon_i=  \eta (v(o_i^+,o_i^-)-v_d(o_i^+,o_i^-))$ does the opposite. If $v(o_i^+,o_i^-) > v_d(o_i^+,o_i^-)$,  a current $\epsilon_i > 0$ increases the pressure drop $v(o_i^+,o_i^-)$ but this takes $v(o_i^+,o_i^-)$ farther from $v_d(o_i^+,o_i^-)$. Therefore we must choose a feedback current $\epsilon_i=  -\eta (v(o_i^+,o_i^-)-v_d(o_i^+,o_i^-))$ which changes the sign of $u(x,y)$. Looking at Eq.~\ref{eq:proof-5}, this modifies our learning rule to $\Delta w_{xy} = -u(x,y)v(x,y)$
    \item We define free and nudged states as $v^{\rm free}(x,y)=v(x,y)$ and $v^{\rm nudged}(x,y)=v(x,y)+u(x,y)$ for all $w_{xy} \in W $. We get a learning rule in terms of free and nudged states as $\Delta w_{xy} =  - u(x,y)v(x,y) = (v^{\rm free}(x,y)-v^{\rm nudged}(x,y))v^{\rm free}(x,y)$.
\end{enumerate}
More generally, the learning rule of equilibrium propagation and coupled learning can be written in terms of derivatives of energy with respect to the trainable parameters\cite{Scellier2017,Stern2021,scellier2020deep}, as follows:
\begin{equation}
    \label{eqprop-rule-general}
    \Delta \mathbf{w} = 2k \bigg( \dfrac{\partial E^{\rm free}}{\partial \mathbf{w}} -  \dfrac{\partial E^{\rm nudged}}{\partial \mathbf{w} } \bigg),
\end{equation}
where $E^{\rm free}$ is the energy function in the free phase and $E^{\rm nudged}$ is the energy function in the nudged phase. The advantage of the above formulation is that it can be used for general systems driven by physical equilibration. For example, Eq~\ref{eqprop-rule-resistive} can be obtained from Eq~\ref{eqprop-rule-general} by taking $E$ as power dissipation function.

We can now rewrite our learning rule in terms of energy:
\begin{align}
 \Delta w_{xy} & = - u(x,y)v(x,y) \\ & =  \dfrac{1}{2}(v(x,y))^2+\dfrac{1}{2}(u(x,y))^2 -\dfrac{1}{2}(v(x,y)+u(x,y))^2  \\
  & =  \dfrac{d U^{In}}{d w_{xy}}  \bigg|_{x=v} + \dfrac{d U^{Fb}}{d w_{xy}}  \bigg|_{x=u} -\dfrac{d U^{In+Fb}}{d w_{xy}}  \bigg|_{x=u+v} \\
               & =  \dfrac{\partial U^{In}}{\partial w_{xy}}  \bigg|_{x=v} + \dfrac{\partial U^{Fb}}{\partial w_{xy}}  \bigg|_{x=u} -\dfrac{\partial U^{In+Fb}}{\partial w_{xy}}  \bigg|_{x=u+v},
\end{align}
where $U(\mathbf{x},\mathbf{w})$ is power dissipation function of potential drops $\mathbf{x}$ and weights $\mathbf{w}$. $U^{In+Fb}$ is the energy function when both the input boundary conditions and feedback boundary conditions are applied simultaneously (similar to nudged state) and $U^{In}$ is the energy function when only input boundary conditions are applied (similar to free state). Note that all the derivatives are evaluated at steady state points, therefore the first order variation of $U$ with respect to the potentials are zero and the total derivatives reduce to partial derivatives. Comparing with Eq~\ref{eqprop-rule-general} we see that there is an extra derivative of $U^{Fb}$ in our equation. This happens because our learning rule is symmetric in feedback and feedforward signals. Our hypothesis is that Eq~\ref{eqprop-rule-general} should work for general energy based models, which we leave for future studies.


Section IV: 
By comparing our model to equilibrium propagation and coupled learning we see that:
\begin{enumerate}
    \item Chemical signals can be used to realize nudged states with the learning rate playing the role of the nudge amplitude.
    \item Using chemical signaling, the system components can now differentiate between ``feedforward'' and ``feedback'' signals. This contrasts with equilibrium propagation and coupled learning, where error signals are encoded in the difference of ``nudged states'' and ``free states''.
    %This opens up the possibility of training via making continuous modifications to the system.
    \item Unlike equilibrium propagation and coupled learning, our model treats feedback and feedforward signals symmetrically.
\end{enumerate} 




\section{Extra points(May not be true , needs further discussion)}

\begin{enumerate}
    \item In this model, instead of segregating the feedback and feed-forward paths(which can be done by using two superimposed networks, similar to experimental work done by Sam Dillanvou), we modify a node to store information of two independent quantities u and v. where v is the feed-forward chemical concentration and u is the feedback chemical concentration. 
    \item One issue with training a physical system is sending signed error information using unsigned physical quantities(like pressure at every node,etc). Eq-prop solves this by using two phases of the network and taking a difference of physical quantities between two phases(probably temporally separated). This way one can get signed local information. In our model this signed error information is locally obtained by taking a difference between physical quantities across the weights. (In our model we are taking a spatially separated difference instead of temporally separated one).
    \item Let $E(x;w,BC_1+BC_2)$ is the power dissipation function of a resistor network with weights w when boundary condition 1 and boundary condition 2 are applied simultaneously. Can we write $E(x;w,BC_1+BC_2)=E(x;w,BC_1)+E(x;w,BC_2)$ ?
    \item Slime mold moves fluid around its body using peristaltic wave motion.  We can use a similar process in our model to make the relationship between input and output pressures nonlinear.
    
    \item It could be possible to make a similar learning mechanism for continuous systems. (Eg; Diffusion equation on a 2d surface with weights analogous to a position dependent diffusion constant).  Slime mold resembles more like a network shaped cut out from a similar continuous learning system.
    
    \item "Equilibrium Propagation requires only one kind of neural computations for both phases of training, making it more biologically plausible than Backpropagation " - what does it mean by one kind of neural computation ? why does it make it more biologically plausible ?
    \item Our learning rule is symmetric in feedforward and feedback signals. Does this mean that fundamentally, external input and internal feedback are of the same nature ?
    \item Where does this model stand in comparison to existing models explaining credit assignment in brain ?
    \item Is this an NGRAD kind of model ?
    \item Is there an explicit top down transfer of error information ?
    \item Because the feedback chemical is released after the pressures at output nodes settle to equilibrium, doesn't it mean there is a separate feedforward and feedback phase even here ?
\end{enumerate}
